Distributionally Robust Chance-Constrained Programs with Right-Hand Side Uncertainty under Wasserstein Ambiguity

We consider exact deterministic mixed-integer programming (MIP) reformulations of distributionally robust chance-constrained programs (DR-CCP) with random right-hand sides over Wasserstein ambiguity sets. The existing MIP formulations are known to have weak continuous relaxation bounds, and, consequently, for hard instances with small radius, or with large problem sizes, the branch-and-bound based solution processes suffer from large optimality gaps even after hours of computation time. This significantly hinders the practical application of the DR-CCP paradigm. Motivated by these challenges, we conduct a polyhedral study to strengthen these formulations. We reveal several hidden connections between DR-CCP and its nominal counterpart (the sample average approximation), mixing sets, and robust 0-1 programming. By exploiting these connections in combination, we provide an improved formulation and two classes of valid inequalities for DR-CCP. We test the impact of our results on a stochastic transportation problem numerically. Our experiments demonstrate the effectiveness of our approach; in particular our improved formulation and proposed valid inequalities reduce the overall solution times remarkably. Moreover, this allows us to significantly scale up the problem sizes that can be handled in such DR-CCP formulations by reducing the solution times from hours to seconds.

==> results_100.tex <==
\begin{landscape}

\begin{table}
	\centering
	\caption{Results for $N=100$, $F=5$, $D=50$, $\epsilon=0.1$}
	\label{tab:full-N100-F5-D50-timegapcuts}
	{\tiny
	\begin{tabular}{l|rr|rr|rrr|rrr|rrr}
		\toprule
		{} & \multicolumn{2}{c}{\texttt{Basic}} & \multicolumn{2}{c}{\texttt{Improved}} & \multicolumn{3}{c}{\texttt{Mixing}} & \multicolumn{3}{c}{\texttt{Path}} & \multicolumn{3}{c}{\texttt{Mixing+Path}} \\
		{} &       Slv(Fnd) & Time(Gap) &          Slv(Fnd) & Time(Gap) &        Slv(Fnd) & Time(Gap) &  Cuts &      Slv(Fnd) & Time(Gap) &   Cuts &             Slv(Fnd) & Time(Gap) &        Cuts \\
		\midrule
		$\theta_{1}$  &          0(10) &   *(1.16) &            10(10) &   4.29(*) &          10(10) &   6.64(*) &  54.7 &        10(10) &   7.31(*) &  287.6 &               10(10) &   8.40(*) &  41.7/274.6 \\
		$\theta_{2}$  &         10(10) &  26.58(*) &            10(10) &   0.04(*) &          10(10) &   0.05(*) &   0.3 &        10(10) &   0.06(*) &   88.2 &               10(10) &   0.06(*) &    0.3/88.2 \\
		$\theta_{3}$  &         10(10) &   4.27(*) &            10(10) &   0.04(*) &          10(10) &   0.04(*) &   0.0 &        10(10) &   0.04(*) &   73.8 &               10(10) &   0.05(*) &    0.0/73.8 \\
		$\theta_{4}$  &         10(10) &   3.36(*) &            10(10) &   0.03(*) &          10(10) &   0.03(*) &   0.0 &        10(10) &   0.03(*) &   44.4 &               10(10) &   0.03(*) &    0.0/44.4 \\
		$\theta_{5}$  &         10(10) &   1.34(*) &            10(10) &   0.03(*) &          10(10) &   0.03(*) &   0.0 &        10(10) &   0.03(*) &   42.4 &               10(10) &   0.03(*) &    0.0/42.4 \\
		$\theta_{6}$  &         10(10) &   1.17(*) &            10(10) &   0.03(*) &          10(10) &   0.03(*) &   0.0 &        10(10) &   0.03(*) &   43.1 &               10(10) &   0.03(*) &    0.0/43.1 \\
		$\theta_{7}$  &         10(10) &   1.04(*) &            10(10) &   0.03(*) &          10(10) &   0.03(*) &   0.0 &        10(10) &   0.03(*) &   40.3 &               10(10) &   0.03(*) &    0.0/40.3 \\
		$\theta_{8}$  &         10(10) &   0.94(*) &            10(10) &   0.03(*) &          10(10) &   0.03(*) &   0.0 &        10(10) &   0.03(*) &   40.2 &               10(10) &   0.03(*) &    0.0/40.2 \\
		$\theta_{9}$  &         10(10) &   0.86(*) &            10(10) &   0.03(*) &          10(10) &   0.03(*) &   0.0 &        10(10) &   0.03(*) &   36.4 &               10(10) &   0.03(*) &    0.0/36.4 \\
		$\theta_{10}$ &         10(10) &   0.84(*) &            10(10) &   0.02(*) &          10(10) &   0.03(*) &   0.0 &        10(10) &   0.03(*) &   36.0 &               10(10) &   0.03(*) &    0.0/36.0 \\
		\bottomrule
	\end{tabular}
	}
\end{table}

\begin{table}
	\centering
	\caption{Results at root node for $N=100$, $F=5$, $D=50$, $\epsilon=0.1$}
	\label{tab:full-N100-F5-D50-root}
	{\tiny
	\begin{tabular}{l|rr|rr|rr|rr|rr}
		\toprule
		{} & \multicolumn{2}{c}{\texttt{Basic}} & \multicolumn{2}{c}{\texttt{Improved}} & \multicolumn{2}{c}{\texttt{Mixing}} & \multicolumn{2}{c}{\texttt{Path}} & \multicolumn{2}{c}{\texttt{Mixing+Path}} \\
		{} &         R.time &  R.gap &            R.time & R.gap &          R.time & R.gap &        R.time & R.gap &               R.time & R.gap \\
		\midrule
		$\theta_{1}$  &           5.67 &  90.53 &              0.19 &  0.34 &            0.21 &  0.35 &          0.50 &  0.31 &                 0.47 &  0.31 \\
		$\theta_{2}$  &          11.22 &  65.19 &              0.04 &  0.00 &            0.05 &  0.00 &          0.06 &  0.00 &                 0.06 &  0.00 \\
		$\theta_{3}$  &           2.98 &  38.94 &              0.04 &  0.00 &            0.04 &  0.00 &          0.04 &  0.00 &                 0.05 &  0.00 \\
		$\theta_{4}$  &           2.66 &  13.35 &              0.03 &  0.00 &            0.03 &  0.00 &          0.03 &  0.00 &                 0.03 &  0.00 \\
		$\theta_{5}$  &           1.32 &   0.04 &              0.03 &  0.00 &            0.03 &  0.00 &          0.03 &  0.00 &                 0.03 &  0.00 \\
		$\theta_{6}$  &           1.17 &   0.00 &              0.03 &  0.00 &            0.03 &  0.00 &          0.03 &  0.00 &                 0.03 &  0.00 \\
		$\theta_{7}$  &           1.04 &   0.00 &              0.03 &  0.00 &            0.03 &  0.00 &          0.03 &  0.00 &                 0.03 &  0.00 \\
		$\theta_{8}$  &           0.94 &   0.00 &              0.03 &  0.00 &            0.03 &  0.00 &          0.03 &  0.00 &                 0.03 &  0.00 \\
		$\theta_{9}$  &           0.86 &   0.00 &              0.03 &  0.00 &            0.03 &  0.00 &          0.03 &  0.00 &                 0.03 &  0.00 \\
		$\theta_{10}$ &           0.84 &   0.00 &              0.02 &  0.00 &            0.03 &  0.00 &          0.03 &  0.00 &                 0.03 &  0.00 \\
		\bottomrule
	\end{tabular}
	}
\end{table}

\end{landscape}




\begin{landscape}

\begin{table}
	\centering
	\caption{Results for $N=100$, $F=10$, $D=100$, $\epsilon=0.1$}
	\label{tab:full-N100-F10-D100-timegapcuts}
	{\tiny
	\begin{tabular}{l|rr|rr|rrr|rrr|rrr}
		\toprule
		{} & \multicolumn{2}{c}{\texttt{Basic}} & \multicolumn{2}{c}{\texttt{Improved}} & \multicolumn{3}{c}{\texttt{Mixing}} & \multicolumn{3}{c}{\texttt{Path}} & \multicolumn{3}{c}{\texttt{Mixing+Path}} \\
		{} &       Slv(Fnd) & Time(Gap) &          Slv(Fnd) & Time(Gap) &        Slv(Fnd) & Time(Gap) &  Cuts &      Slv(Fnd) & Time(Gap) &   Cuts &             Slv(Fnd) & Time(Gap) &        Cuts \\
		\midrule
		$\theta_{1}$  &          0(10) &   *(3.01) &            10(10) &  10.46(*) &          10(10) &  19.19(*) &  55.7 &        10(10) &  29.36(*) &  228.2 &               10(10) &  35.45(*) &  48.0/236.2 \\
		$\theta_{2}$  &         10(10) &  37.49(*) &            10(10) &   0.11(*) &          10(10) &   0.11(*) &   0.0 &        10(10) &   0.12(*) &  171.3 &               10(10) &   0.13(*) &   0.0/171.3 \\
		$\theta_{3}$  &         10(10) &  18.45(*) &            10(10) &   0.10(*) &          10(10) &   0.10(*) &   0.0 &        10(10) &   0.11(*) &  146.7 &               10(10) &   0.12(*) &   0.0/146.7 \\
		$\theta_{4}$  &         10(10) &  16.91(*) &            10(10) &   0.09(*) &          10(10) &   0.09(*) &   0.0 &        10(10) &   0.10(*) &  123.2 &               10(10) &   0.10(*) &   0.0/123.2 \\
		$\theta_{5}$  &         10(10) &   9.17(*) &            10(10) &   0.09(*) &          10(10) &   0.09(*) &   0.0 &        10(10) &   0.09(*) &  119.0 &               10(10) &   0.09(*) &   0.0/119.0 \\
		$\theta_{6}$  &         10(10) &   5.71(*) &            10(10) &   0.06(*) &          10(10) &   0.06(*) &   0.0 &        10(10) &   0.07(*) &   84.7 &               10(10) &   0.07(*) &    0.0/84.7 \\
		$\theta_{7}$  &         10(10) &   4.74(*) &            10(10) &   0.06(*) &          10(10) &   0.06(*) &   0.0 &        10(10) &   0.07(*) &   86.3 &               10(10) &   0.07(*) &    0.0/86.3 \\
		$\theta_{8}$  &         10(10) &   3.78(*) &            10(10) &   0.06(*) &          10(10) &   0.06(*) &   0.0 &        10(10) &   0.07(*) &   74.5 &               10(10) &   0.07(*) &    0.0/74.5 \\
		$\theta_{9}$  &         10(10) &   3.20(*) &            10(10) &   0.06(*) &          10(10) &   0.06(*) &   0.0 &        10(10) &   0.06(*) &   69.9 &               10(10) &   0.06(*) &    0.0/69.9 \\
		$\theta_{10}$ &         10(10) &   2.89(*) &            10(10) &   0.05(*) &          10(10) &   0.06(*) &   0.0 &        10(10) &   0.06(*) &   54.8 &               10(10) &   0.06(*) &    0.0/54.8 \\
		\bottomrule
	\end{tabular}
	}
\end{table}

\begin{table}
	\centering
	\caption{Results at root node for $N=100$, $F=10$, $D=100$, $\epsilon=0.1$}
	\label{tab:full-N100-F10-D100-root}
	{\tiny
	\begin{tabular}{l|rr|rr|rr|rr|rr}
		\toprule
		{} & \multicolumn{2}{c}{\texttt{Basic}} & \multicolumn{2}{c}{\texttt{Improved}} & \multicolumn{2}{c}{\texttt{Mixing}} & \multicolumn{2}{c}{\texttt{Path}} & \multicolumn{2}{c}{\texttt{Mixing+Path}} \\
		{} &         R.time &  R.gap &            R.time & R.gap &          R.time & R.gap &        R.time & R.gap &               R.time & R.gap \\
		\midrule
		$\theta_{1}$  &          29.20 &  90.99 &              0.38 &  0.42 &            0.35 &  0.44 &          0.46 &  0.43 &                 0.50 &  0.43 \\
		$\theta_{2}$  &          10.39 &  68.59 &              0.11 &  0.00 &            0.11 &  0.00 &          0.12 &  0.00 &                 0.13 &  0.00 \\
		$\theta_{3}$  &          14.11 &  43.85 &              0.10 &  0.00 &            0.10 &  0.00 &          0.11 &  0.00 &                 0.12 &  0.00 \\
		$\theta_{4}$  &          14.50 &  21.52 &              0.09 &  0.00 &            0.09 &  0.00 &          0.10 &  0.00 &                 0.10 &  0.00 \\
		$\theta_{5}$  &           8.97 &   1.12 &              0.09 &  0.00 &            0.09 &  0.00 &          0.09 &  0.00 &                 0.09 &  0.00 \\
		$\theta_{6}$  &           5.66 &   0.01 &              0.06 &  0.00 &            0.06 &  0.00 &          0.07 &  0.00 &                 0.07 &  0.00 \\
		$\theta_{7}$  &           4.76 &   0.01 &              0.06 &  0.00 &            0.06 &  0.00 &          0.07 &  0.00 &                 0.07 &  0.00 \\
		$\theta_{8}$  &           3.78 &   0.00 &              0.06 &  0.00 &            0.06 &  0.00 &          0.07 &  0.00 &                 0.07 &  0.00 \\
		$\theta_{9}$  &           3.20 &   0.00 &              0.06 &  0.00 &            0.06 &  0.00 &          0.06 &  0.00 &                 0.06 &  0.00 \\
		$\theta_{10}$ &           2.89 &   0.01 &              0.05 &  0.00 &            0.06 &  0.00 &          0.06 &  0.00 &                 0.06 &  0.00 \\
		\bottomrule
	\end{tabular}
	}
\end{table}

\end{landscape}

==> results_1000.tex <==
\begin{landscape}

\begin{table}
	\centering
	\caption{Results for $N=1000$, $F=5$, $D=50$, $\epsilon=0.1$}
	\label{tab:full-N1000-F5-D50-timegapcuts}
	{\tiny
	\begin{tabular}{l|rr|rr|rrr|rrr|rrr}
		\toprule
		{} & \multicolumn{2}{c}{\texttt{Basic}} & \multicolumn{2}{c}{\texttt{Improved}} & \multicolumn{3}{c}{\texttt{Mixing}} & \multicolumn{3}{c}{\texttt{Path}} & \multicolumn{3}{c}{\texttt{Mixing+Path}} \\
		{} &       Slv(Fnd) &  Time(Gap) &          Slv(Fnd) & Time(Gap) &        Slv(Fnd) & Time(Gap) &   Cuts &      Slv(Fnd) & Time(Gap) &    Cuts &             Slv(Fnd) & Time(Gap) &          Cuts \\
		\midrule
		$\theta_{1}$  &           0(6) &   *(97.90) &             0(10) &   *(0.59) &           0(10) &   *(0.52) &  532.8 &         0(10) &   *(0.44) &  2472.5 &                0(10) &   *(0.44) &  381.0/2377.9 \\
		$\theta_{2}$  &          0(10) &   *(66.04) &            10(10) &  36.84(*) &          10(10) &  36.68(*) &    0.0 &        10(10) &  40.41(*) &   114.3 &               10(10) &  40.61(*) &     0.0/114.3 \\
		$\theta_{3}$  &          0(10) &   *(31.10) &            10(10) &   9.15(*) &          10(10) &   9.33(*) &    0.0 &        10(10) &   9.23(*) &    82.9 &               10(10) &   9.61(*) &      0.0/82.9 \\
		$\theta_{4}$  &          0(10) &    *(2.11) &            10(10) &   7.73(*) &          10(10) &   7.60(*) &    0.0 &        10(10) &   7.74(*) &    61.6 &               10(10) &   7.71(*) &      0.0/61.6 \\
		$\theta_{5}$  &         10(10) &  287.92(*) &            10(10) &   6.12(*) &          10(10) &   6.16(*) &    0.0 &        10(10) &   6.20(*) &    58.5 &               10(10) &   6.19(*) &      0.0/58.5 \\
		$\theta_{6}$  &         10(10) &  130.38(*) &            10(10) &   5.83(*) &          10(10) &   5.83(*) &    0.0 &        10(10) &   5.95(*) &    49.0 &               10(10) &   5.94(*) &      0.0/49.0 \\
		$\theta_{7}$  &         10(10) &  117.77(*) &            10(10) &   5.75(*) &          10(10) &   5.72(*) &    0.0 &        10(10) &   5.77(*) &    48.9 &               10(10) &   5.75(*) &      0.0/48.9 \\
		$\theta_{8}$  &         10(10) &   99.95(*) &            10(10) &   5.58(*) &          10(10) &   5.52(*) &    0.0 &        10(10) &   5.65(*) &    49.0 &               10(10) &   5.64(*) &      0.0/49.0 \\
		$\theta_{9}$  &         10(10) &   90.82(*) &            10(10) &   5.27(*) &          10(10) &   5.27(*) &    0.0 &        10(10) &   5.34(*) &    49.0 &               10(10) &   5.39(*) &      0.0/49.0 \\
		$\theta_{10}$ &         10(10) &   78.88(*) &            10(10) &   4.95(*) &          10(10) &   4.97(*) &    0.0 &        10(10) &   5.04(*) &    49.1 &               10(10) &   5.02(*) &      0.0/49.1 \\
		\bottomrule
	\end{tabular}
	}
\end{table}

\begin{table}
	\centering
	\caption{Results at root node for $N=1000$, $F=5$, $D=50$, $\epsilon=0.1$}
	\label{tab:full-N1000-F5-D50-root}
	{\tiny
	\begin{tabular}{l|rr|rr|rr|rr|rr}
		\toprule
		{} & \multicolumn{2}{c}{\texttt{Basic}} & \multicolumn{2}{c}{\texttt{Improved}} & \multicolumn{2}{c}{\texttt{Mixing}} & \multicolumn{2}{c}{\texttt{Path}} & \multicolumn{2}{c}{\texttt{Mixing+Path}} \\
		{} &         R.time &  R.gap &            R.time & R.gap &          R.time & R.gap &        R.time & R.gap &               R.time & R.gap \\
		\midrule
		$\theta_{1}$  &        2334.91 &  99.45 &            338.01 &  0.63 &          614.52 &  0.54 &       1968.43 &  0.45 &              2000.91 &  0.45 \\
		$\theta_{2}$  &         275.76 &  73.64 &             37.57 &  0.01 &           36.76 &  0.01 &         40.65 &  0.00 &                40.48 &  0.00 \\
		$\theta_{3}$  &         223.92 &  47.13 &              9.22 &  0.00 &            9.30 &  0.00 &          9.29 &  0.00 &                 9.59 &  0.00 \\
		$\theta_{4}$  &         289.21 &  16.30 &              7.70 &  0.00 &            7.71 &  0.00 &          7.77 &  0.00 &                 7.77 &  0.00 \\
		$\theta_{5}$  &         103.41 &   0.51 &              6.10 &  0.00 &            6.09 &  0.00 &          6.19 &  0.00 &                 6.18 &  0.00 \\
		$\theta_{6}$  &          89.56 &   0.39 &              5.81 &  0.01 &            5.83 &  0.01 &          5.92 &  0.01 &                 5.86 &  0.01 \\
		$\theta_{7}$  &          78.75 &   0.41 &              5.76 &  0.00 &            5.71 &  0.00 &          5.74 &  0.00 &                 5.80 &  0.00 \\
		$\theta_{8}$  &          67.40 &   0.40 &              5.53 &  0.00 &            5.55 &  0.00 &          5.62 &  0.00 &                 5.65 &  0.00 \\
		$\theta_{9}$  &          63.73 &   0.38 &              5.28 &  0.00 &            5.26 &  0.00 &          5.35 &  0.00 &                 5.36 &  0.00 \\
		$\theta_{10}$ &          58.08 &   0.36 &              4.93 &  0.00 &            4.91 &  0.00 &          5.04 &  0.00 &                 5.03 &  0.00 \\
		\bottomrule
	\end{tabular}
	}
\end{table}

\end{landscape}




\begin{landscape}

\begin{table}
	\centering
	\caption{Results for $N=1000$, $F=10$, $D=100$, $\epsilon=0.1$}
	\label{tab:full-N1000-F10-D100-timegapcuts}
	{\tiny
	\begin{tabular}{l|rr|rr|rrr|rrr|rrr}
		\toprule
		{} & \multicolumn{2}{c}{\texttt{Basic}} & \multicolumn{2}{c}{\texttt{Improved}} & \multicolumn{3}{c}{\texttt{Mixing}} & \multicolumn{3}{c}{\texttt{Path}} & \multicolumn{3}{c}{\texttt{Mixing+Path}} \\
		{} &       Slv(Fnd) &      Time(Gap) &          Slv(Fnd) & Time(Gap) &        Slv(Fnd) & Time(Gap) &   Cuts &      Slv(Fnd) & Time(Gap) &    Cuts &             Slv(Fnd) & Time(Gap) &          Cuts \\
		\midrule
		$\theta_{1}$  &           0(1) &       *(98.73) &             0(10) &   *(0.45) &           0(10) &   *(0.42) &  382.3 &         0(10) &   *(0.39) &  2150.7 &                0(10) &   *(0.39) &  249.6/2032.4 \\
		$\theta_{2}$  &           0(7) &       *(67.05) &            10(10) &  27.02(*) &          10(10) &  26.05(*) &    0.0 &        10(10) &  37.06(*) &   399.8 &               10(10) &  36.97(*) &     0.0/399.8 \\
		$\theta_{3}$  &           0(4) &       *(34.22) &            10(10) &  14.44(*) &          10(10) &  14.73(*) &    0.0 &        10(10) &  15.55(*) &   231.1 &               10(10) &  14.70(*) &     0.0/231.1 \\
		$\theta_{4}$  &           0(5) &       *(10.48) &            10(10) &  10.18(*) &          10(10) &  10.41(*) &    0.0 &        10(10) &  12.13(*) &   186.3 &               10(10) &  12.07(*) &     0.0/186.3 \\
		$\theta_{5}$  &          4(10) &  2599.60(0.45) &            10(10) &  10.37(*) &          10(10) &  10.68(*) &    0.0 &        10(10) &  11.66(*) &   186.1 &               10(10) &  11.31(*) &     0.0/186.1 \\
		$\theta_{6}$  &         10(10) &      968.46(*) &            10(10) &   3.14(*) &          10(10) &   3.25(*) &    0.0 &        10(10) &   3.29(*) &    96.3 &               10(10) &   3.28(*) &      0.0/96.3 \\
		$\theta_{7}$  &         10(10) &      853.68(*) &            10(10) &   2.91(*) &          10(10) &   3.06(*) &    0.0 &        10(10) &   3.48(*) &    96.4 &               10(10) &   3.52(*) &      0.0/96.4 \\
		$\theta_{8}$  &         10(10) &      647.80(*) &            10(10) &   3.08(*) &          10(10) &   3.11(*) &    0.0 &        10(10) &   3.12(*) &    96.3 &               10(10) &   3.07(*) &      0.0/96.3 \\
		$\theta_{9}$  &         10(10) &      528.73(*) &            10(10) &   2.78(*) &          10(10) &   2.74(*) &    0.0 &        10(10) &   2.81(*) &    96.2 &               10(10) &   2.85(*) &      0.0/96.2 \\
		$\theta_{10}$ &         10(10) &      375.32(*) &            10(10) &   2.58(*) &          10(10) &   2.57(*) &    0.0 &        10(10) &   2.60(*) &    96.5 &               10(10) &   2.59(*) &      0.0/96.5 \\
		\bottomrule
	\end{tabular}
	}
\end{table}

\begin{table}
	\centering
	\caption{Results at root node for $N=1000$, $F=10$, $D=100$, $\epsilon=0.1$}
	\label{tab:full-N1000-F10-D100-root}
	{\tiny
	\begin{tabular}{l|rr|rr|rr|rr|rr}
		\toprule
		{} & \multicolumn{2}{c}{\texttt{Basic}} & \multicolumn{2}{c}{\texttt{Improved}} & \multicolumn{2}{c}{\texttt{Mixing}} & \multicolumn{2}{c}{\texttt{Path}} & \multicolumn{2}{c}{\texttt{Mixing+Path}} \\
		{} &         R.time &  R.gap &            R.time & R.gap &          R.time & R.gap &        R.time & R.gap &               R.time & R.gap \\
		\midrule
		$\theta_{1}$  &        3542.86 &  99.48 &             29.81 &  0.50 &           35.95 &  0.45 &        148.13 &  0.41 &               157.22 &  0.41 \\
		$\theta_{2}$  &        1185.36 &  72.76 &             27.02 &  0.01 &           26.05 &  0.01 &         37.06 &  0.00 &                36.97 &  0.00 \\
		$\theta_{3}$  &         990.87 &  46.39 &             14.44 &  0.01 &           14.73 &  0.01 &         15.55 &  0.01 &                14.70 &  0.01 \\
		$\theta_{4}$  &        1547.07 &  21.38 &             10.18 &  0.01 &           10.41 &  0.01 &         12.13 &  0.00 &                12.07 &  0.00 \\
		$\theta_{5}$  &         570.64 &   0.84 &             10.37 &  0.00 &           10.68 &  0.00 &         11.66 &  0.00 &                11.31 &  0.00 \\
		$\theta_{6}$  &         498.69 &   0.41 &              3.14 &  0.00 &            3.25 &  0.00 &          3.29 &  0.00 &                 3.28 &  0.00 \\
		$\theta_{7}$  &         453.85 &   0.43 &              2.91 &  0.00 &            3.06 &  0.00 &          3.48 &  0.00 &                 3.52 &  0.00 \\
		$\theta_{8}$  &         412.37 &   0.40 &              3.08 &  0.00 &            3.11 &  0.00 &          3.12 &  0.00 &                 3.07 &  0.00 \\
		$\theta_{9}$  &         366.56 &   0.36 &              2.78 &  0.00 &            2.74 &  0.00 &          2.81 &  0.00 &                 2.85 &  0.00 \\
		$\theta_{10}$ &         314.52 &   0.25 &              2.58 &  0.00 &            2.57 &  0.00 &          2.60 &  0.00 &                 2.59 &  0.00 \\
		\bottomrule
	\end{tabular}
	}
\end{table}

\end{landscape}

==> results_3000.tex <==
\begin{landscape}
\begin{table}
	\centering
	\caption{Results for $N=3000$, $F=5$, $D=50$, $\epsilon=0.1$}
	\label{tab:full-N3000-timegapcuts}
	{\tiny
	\begin{tabular}{l|rr|rr|rrr|rrr|rrr}
		\toprule
		{} & \multicolumn{2}{c}{\texttt{Basic}} & \multicolumn{2}{c}{\texttt{Improved}} & \multicolumn{3}{c}{\texttt{Mixing}} & \multicolumn{3}{c}{\texttt{Path}} & \multicolumn{3}{c}{\texttt{Mixing+Path}} \\
		{} &       Slv(Fnd) & Time(Gap) &          Slv(Fnd) & Time(Gap) &        Slv(Fnd) & Time(Gap) &    Cuts &      Slv(Fnd) & Time(Gap) &    Cuts &             Slv(Fnd) & Time(Gap) &           Cuts \\
		\midrule
		$\theta_{1}$  &           0(0) &       n/a &             0(10) &   *(0.78) &           0(10) &   *(0.52) &  2358.2 &         0(10) &   *(0.62) &  6536.0 &                0(10) &   *(0.48) &  1470.3/4228.1 \\
		$\theta_{2}$  &           0(5) &  *(69.56) &             0(10) &   *(0.49) &           0(10) &   *(0.49) &     0.0 &         0(10) &   *(0.41) &  6324.6 &                0(10) &   *(0.41) &     0.0/6102.2 \\
		$\theta_{3}$  &           0(4) &  *(48.65) &            10(10) &  17.89(*) &          10(10) &  17.62(*) &     0.0 &        10(10) &  18.94(*) &   200.8 &               10(10) &  18.29(*) &      0.0/200.8 \\
		$\theta_{4}$  &           0(4) &  *(15.01) &            10(10) &  13.74(*) &          10(10) &  13.22(*) &     0.0 &        10(10) &  14.03(*) &    94.1 &               10(10) &  13.94(*) &       0.0/94.1 \\
		$\theta_{5}$  &          0(10) &   *(1.11) &            10(10) &  12.75(*) &          10(10) &  12.60(*) &     0.0 &        10(10) &  13.65(*) &    88.3 &               10(10) &  13.55(*) &       0.0/88.3 \\
		$\theta_{6}$  &          0(10) &   *(0.58) &            10(10) &  12.29(*) &          10(10) &  12.21(*) &     0.0 &        10(10) &  12.83(*) &    80.2 &               10(10) &  12.68(*) &       0.0/80.2 \\
		$\theta_{7}$  &          0(10) &   *(0.48) &            10(10) &  12.28(*) &          10(10) &  12.01(*) &     0.0 &        10(10) &  12.93(*) &    56.7 &               10(10) &  12.95(*) &       0.0/56.7 \\
		$\theta_{8}$  &          0(10) &   *(0.40) &            10(10) &  12.48(*) &          10(10) &  12.20(*) &     0.0 &        10(10) &  12.78(*) &    52.9 &               10(10) &  12.65(*) &       0.0/52.9 \\
		$\theta_{9}$  &          0(10) &   *(0.37) &            10(10) &  11.96(*) &          10(10) &  11.81(*) &     0.0 &        10(10) &  12.36(*) &    49.4 &               10(10) &  12.52(*) &       0.0/49.4 \\
		$\theta_{10}$ &          0(10) &   *(0.28) &            10(10) &   8.04(*) &          10(10) &   8.19(*) &     0.0 &        10(10) &   8.86(*) &    49.4 &               10(10) &   8.94(*) &       0.0/49.4 \\
		\bottomrule
	\end{tabular}
	}
\end{table}

\begin{table}
	\centering
	\caption{Results at root node for $N=3000$, $F=5$, $D=50$, $\epsilon=0.1$}
	\label{tab:full-N3000-root}
	{\tiny
	\begin{tabular}{l|rr|rr|rr|rr|rr}
		\toprule
		{} & \multicolumn{2}{c}{\texttt{Basic}} & \multicolumn{2}{c}{\texttt{Improved}} & \multicolumn{2}{c}{\texttt{Mixing}} & \multicolumn{2}{c}{\texttt{Path}} & \multicolumn{2}{c}{\texttt{Mixing+Path}} \\
		{} &         R.time &  R.gap &            R.time & R.gap &          R.time & R.gap &        R.time & R.gap &               R.time & R.gap \\
		\midrule
		$\theta_{1}$  &            n/a &    n/a &             72.08 &  0.80 &         1931.99 &  0.52 &       3598.81 &  0.62 &              3601.05 &  0.48 \\
		$\theta_{2}$  &        3144.09 &  70.41 &            134.46 &  0.55 &          109.72 &  0.55 &       3600.10 &  0.41 &              3600.22 &  0.41 \\
		$\theta_{3}$  &        2952.26 &  51.31 &             17.89 &  0.01 &           17.62 &  0.01 &         18.94 &  0.01 &                18.29 &  0.01 \\
		$\theta_{4}$  &        2684.77 &  15.72 &             13.74 &  0.01 &           13.22 &  0.01 &         14.03 &  0.01 &                13.94 &  0.01 \\
		$\theta_{5}$  &        3181.43 &   1.14 &             12.75 &  0.00 &           12.60 &  0.00 &         13.65 &  0.00 &                13.55 &  0.00 \\
		$\theta_{6}$  &        3176.11 &   0.63 &             12.29 &  0.00 &           12.21 &  0.00 &         12.83 &  0.00 &                12.68 &  0.00 \\
		$\theta_{7}$  &        2958.81 &   0.55 &             12.28 &  0.01 &           12.01 &  0.01 &         12.93 &  0.01 &                12.95 &  0.01 \\
		$\theta_{8}$  &        2876.49 &   0.47 &             12.48 &  0.01 &           12.20 &  0.01 &         12.78 &  0.01 &                12.65 &  0.01 \\
		$\theta_{9}$  &        2781.77 &   0.45 &             11.96 &  0.01 &           11.81 &  0.01 &         12.36 &  0.01 &                12.52 &  0.01 \\
		$\theta_{10}$ &        2439.69 &   0.41 &              8.04 &  0.01 &            8.19 &  0.01 &          8.86 &  0.01 &                 8.94 &  0.01 \\
		\bottomrule
	\end{tabular}
	}
\end{table}
\end{landscape}
